A robust solution strategy for the Cahn-Larch\'e equations

In this paper we propose a solution strategy for the Cahn-Larch\'e equations, which is a model for linearized elasticity in a medium with two elastic phases that evolve subject to a Ginzburg-Landau type energy functional. The system can be seen as a combination of the Cahn-Hilliard regularized interface equation and linearized elasticity, and is non-linearly coupled, has a fourth order term that comes from the Cahn-Hilliard subsystem, and is non-convex and nonlinear in both the phase-field and displacement variables. We propose a novel semi-implicit discretization in time that uses a standard convex-concave splitting method of the nonlinear double-well potential, as well as special treatment to the elastic energy. We show that the resulting discrete system is equivalent to a convex minimization problem, and propose and prove the convergence of alternating minimization applied to it. Finally, we present numerical experiments that show the robustness and effectiveness of both alternating minimization and the monolithic Newton method applied to the newly proposed discrete system of equations. We compare it to a system of equations that has been discretized with a standard convex-concave splitting of the double-well potential, and implicit evaluations of the elasticity contributions and show that the newly proposed discrete system is better conditioned for linearization techniques.

==> circlesfig.tex <==
\begin{figure}
\centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-smallgamma0.png}
        \caption{$t = 0$}
        \label{fig:circlessg0}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-smallgamma100.png}
        \caption{$t = 0.001$}
        \label{fig:circlessg100}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-smallgamma500.png}
        \caption{$t = 0.005$}
        \label{fig:circlessg500}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-smallgamma1000.png}
        \caption{$t = 0.01$}
        \label{fig:circlessg1000}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-midgamma0.png}
        \caption{$t = 0$}
        \label{fig:circlesmg0}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-midgamma100.png}
        \caption{$t = 0.001$}
        \label{fig:circlesmg100}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-midgamma500.png}
        \caption{$t = 0.005$}
        \label{fig:circlesmg500}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width = \textwidth]{figs/circles-midgamma1000.png}
        \caption{$t = 0.01$}
        \label{fig:circlesmg1000}
    \end{subfigure}
\label{fig:CHB}
        \hspace{0cm}\includegraphics[width=\textwidth]{figs/colorbarhorizontal.png}
       \caption{(a) -- (l): the solution at time $t$ for the phase-field $\pf$. (a) -- (d): Cahn-Hilliard-Biot with $p=0.25$ on the top, (e) -- (h): Cahn-Hilliard-Biot with zero pressure BC, (i) -- (l): Cahn-Larch\'e. (m): system energy (with external contributions). PD is Cahn-Hilliard-Biot with $p=0.25$ on the top, CHB is Cahn-Hilliard-Biot with zero pressure BC and CHE is Cahn-Larch\'e.}
\end{figure}

==> leftovers.tex <==

From standard theory of linearized elasticity and Cahn-Hilliard both \eqref{eq:min1} and \eqref{eq:min2} have unique minimizers. Let $\langle\cdot ,\cdot\rangle$ be the duality pairing and consider the optimality condition of the first  
\begin{equation}\label{eq:opt1}
\langle \delta_\pf\mathcal{H}^n(\pf_h^{n,i},\bm u_h^{n,i-1}),\eta_h\rangle = 0,
\end{equation}
and the second 
\begin{equation}\label{eq:opt2}
    \langle \delta_{\bm u}\mathcal{H}^n(\pf^{n,i}_h,\bm u^{n,i}_h),\bm v_h\rangle = 0
\end{equation}
minimization problem. Here, $\delta_\pf\mathcal{H}^n$ and $\delta_{\bm u}\mathcal{H}^n$ represent the variational derivative to the first and second argument of $\mathcal{H}^n$, respectively.
Subtract \eqref{eq:opt1} at iteration $i-1$ from \eqref{eq:opt1} at iteration $i$ and test with $\eta_h = \pf^{n,i}_h-\pf^{n,i}_h$ to obtain
\begin{equation*}
    \langle \delta_\pf \mathcal{H}^n(\pf^{n,i}_h,\bm u_h^{n,i-1})-\delta_\pf \mathcal{H}
    ^n(\pf^{n,i-1}_h,\bm u_h^{n,i-2}),\pf_h^{n,i}-\pf_h^{n,i-1}\rangle = 0
\end{equation*}
this is equivalent (by an addition of zero) to
\begin{eqnarray*}
   & \langle \delta_\pf \mathcal{H}^n(\pf^{n,i}_h,\bm u_h^{n,i-1})-\delta_\pf \mathcal{H}
    ^n(\pf^{n,i-1}_h,\bm u_h^{n,i-1}),\pf_h^{n,i}-\pf_h^{n,i-1}\rangle\\
    &=
    \langle \delta_\pf \mathcal{H}^n(\pf^{n,i-1}_h,\bm u_h^{n,i-1})-\delta_\pf \mathcal{H}
    ^n(\pf^{n,i-1}_h,\bm u_h^{n,i-2}),\pf_h^{n,i}-\pf_h^{n,i-1}\rangle 
\end{eqnarray*}
We have that
\begin{eqnarray*}
\langle \delta_\pf \mathcal{H}^n(\pf^{n,i}_h,\bm u_h^{n,i-1})-\delta_\pf \mathcal{H}
    ^n(\pf^{n,i-1}_h,\bm u_h^{n,i-1}),\pf_h^{n,i}-\pf_h^{n,i-1}\rangle &\geq& \| \pf_h^{n,i} - \pf_h^{n,i-1}\|^2_{H^{-1}_m(\Omega)}\\
    && +c_\mathbb{C}\| \pf_h^{n,i} - \pf_h^{n,i-1}\|^2_{L^2(\Omega)}\\
    && + \gamma\| \nabla\left(\pf_h^{n,i} - \pf_h^{n,i-1}\right)\|^2
\end{eqnarray*}
and
\begin{eqnarray*}
    &\langle \delta_\pf \mathcal{H}^n(\pf^{n,i-1}_h,\bm u_h^{n,i-1})-\delta_\pf \mathcal{H}
    ^n(\pf^{n,i-1}_h,\bm u_h^{n,i-2}),\pf_h^{n,i}-\pf_h^{n,i-1}\rangle \\
    & = \left\langle \mathbb{C}\left(\bm\varepsilon(\bm u_h^{n,i-1}) - \bm \varepsilon(\bm u_h^{n,i-2})\right),\pf_h^{n,i}-\pf_h^{n,i-1}\right\rangle_{L^2(\Omega)}\leq C_\mathbb{C}\|\bm\varepsilon(\bm u_h^{n,i-1}) - \bm \varepsilon(\bm u_h^{n,i-2})\|_{L^2(\Omega)}\|\pf_h^{n,i}-\pf_h^{n,i-1}\|_{L^2(\Omega)}
\end{eqnarray*}
In total, we then have that
\begin{equation}
    c_\mathbb{C}\|\pf_h^{n,i} - \pf_h^{n,i-1}\|_{L^2(\Omega)}\leq C_\mathbb{C}\|\bm\varepsilon(\bm u_h^{n,i-1}) - \bm \varepsilon(\bm u_h^{n,i-2})\|_{L^2(\Omega)}.
\end{equation}
Similarly, from \eqref{eq:opt2} we can obtain the estimate
\begin{equation}
    c_\mathbb{C}\|\bm\varepsilon(\bm u_h^{n,i}) - \bm \varepsilon(\bm u_h^{n,i-1})\|_{L^2(\Omega)}\leq  \xi C_\mathbb{C}\|\pf_h^{n,i} - \pf_h^{n,i-1}\|_{L^2(\Omega)}.
\end{equation}
Using the estimates together, we get that $\{pf$


% We now use Cauchy Schwarz' and  Young's inequalities to obtain
% \begin{equation}
%   2\left\langle\mathbb{C}\left(\bm\varepsilon(\bm w_h)\right),\xi s_h\bm I \right\rangle_{L^2(\Omega)}\leq \delta C_\mathbb{C}^2\|\bm \varepsilon(\bm w_h)\|^2_{L^2(\Omega)} + \frac{k}{\delta}\|s_h\|_{L^2(\Omega)}^2 + \frac{1-k}{\delta}\|s_h\|_{L^2(\Omega)}^2
% \end{equation}
% where $\delta>0$ and $1\geq k\geq0$ are free to be chosen paramteters. Using Lemma~\ref{lem:inverseinequality}  we then get
% \begin{equation}
%   2\left\langle\mathbb{C}\left(\bm\varepsilon(\bm w_h)\right),\xi s_h\bm I \right\rangle_{L^2(\Omega)}\leq \delta C_\mathbb{C}^2\|\bm \varepsilon(\bm w_h)\|^2_{L^2(\Omega)} + \frac{k}{\delta}C_{\mathrm{inv}}h^{-1}\|s_h\|_{H^{-1}_m(\Omega)}^2  +\frac{1-k}{\delta}\|s_h\|_{L^2(\Omega)}^2
% \end{equation}
% Therefore, we have 
% \begin{eqnarray}
%      \|(s_h,\bm w_h)\|^2 &\geq& \frac{\|s_h\|_{H^{-1}_m(\Omega)}}{\tau} + \gamma\|\nabla s_h\|^2_{L^2(\Omega)} +  c_\mathbb{C}\|\bm\varepsilon(\bm w_h)\|^2_{L^2(\Omega)}+ \xi^2\bm I:\mathbb{C}\bm I\|s_h\|^2_{L^2(\Omega)}\\
%      && -\delta C_\mathbb{C}^2\|\bm \varepsilon(\bm w_h)\|^2_{L^2(\Omega)} - \frac{k}{\delta}C_{\mathrm{inv}}h^{-1}\|s_h\|_{H^{-1}_m(\Omega)}^2-\frac{1-k}{\delta}\|s_h\|_{L^2(\Omega)}^2\\
%      &=&\left(\frac{1}{\tau}-\frac{k}{\delta}C_{\mathrm{inv}}h^{-1}\right)\|s_h\|_{H^{-1}_m(\Omega)} + \gamma\|\nabla s_h\|^2_{L^2(\Omega)} +  \left(c_\mathbb{C}-\delta C_\mathbb{C}^2\right)\|\bm\varepsilon(\bm w_h)\|^2_{L^2(\Omega)}\\
%      &&+ \left(\xi^2\bm I:\mathbb{C}\bm I-\frac{1-k}{\delta}\right)\|s_h\|^2_{L^2(\Omega)} 
% \end{eqnarray}
% Choosing $\delta = \frac{c_\mathbb{C}}{C_\mathbb{C}^2}$ we get 


% \begin{eqnarray}
%      \|(s_h,\bm w_h)\|^2&\geq&\left(\frac{1}{\tau}-\frac{kC_\mathbb{C}^2C_{\mathrm{inv}}}{c_\mathbb{C}h}\right)\|s_h\|_{H^{-1}_m(\Omega)} + \gamma\|\nabla s_h\|^2_{L^2(\Omega)} + \left(\xi^2\bm I:\mathbb{C}\bm  I-\frac{\left(1-k\right)C_\mathbb{C}^2}{c_\mathbb{C}}\right)\|s_h\|^2_{L^2(\Omega)} \\
%      && +\beta_\mathrm{ch}\|s_h\|^2_\mathrm{ch}-\beta_\mathrm{ch}\|s_h\|^2_\mathrm{ch}
% \end{eqnarray}

% \begin{equation}
%     \left(\frac{1}{\tau}-\frac{kC_\mathbb{C}^2C_{\mathrm{inv}}}{c_\mathbb{C}h}-\frac{\beta_\mathrm{ch}}{\tau}\right) \geq 0 \implies   \left(\frac{1}{\tau}-\frac{kC_\mathbb{C}^2C_{\mathrm{inv}}}{c_\mathbb{C}h}\right)\geq\frac{\beta_\mathrm{ch}}{\tau}\implies
% \end{equation}
% \todo[inline]{Talk with Jakub/Florin about the Cauchy-Schwarz inequality in the above todobox and finish this part of the proof. It will be similar for the bound from below with $\|\bm w_h\|_\mathrm{e}$}


\subsection{Practical solution strategy}
Highlight that it would be the same for the gradient flow convex concave method.
Discuss the use of newton method (only one iteration?) in the Cahn-Hilliard subsystem.
Propose a combination (first the scheme that we know converges and use it in some iterations before switching to Newton (monolithic?) on full problem.

\section{Convergence of splitting method for homogeneous material parameters}
Here, we prove that the proposed splitting method for the homogeneous \eqref{eq:splitch1}--\eqref{eq:splitelastic} converges in each time step, under certain conditions on the material parameters.

\begin{theorem}
Let the chemical mobility be independent on $\pf$, $m(\pf) = m$.
 Define the iteration error functions $e_\pf^{n,i}:=\pf^{n} - \pf^{n,i}$, $ e_\mu^{n,i}: \mu^{n} - \mu^{n,i}$, and $\bm e_{\bm u}^{n,i}:= \bm u^n - \bm u^{n,i}$. Then the scheme \eqref{eq:splitch1}--\eqref{eq:splitelastic} converges for $L\geq  \frac{C_\mathbb{C}^3}{4Cc_\mathbb{C}^2}$ with rate of convergence for the phase-field error 
 \begin{equation}
\|e_\pf^{n,i}\|^2 \leq \frac{L}{\frac{2\gamma}{C_\Omega}+L}\|e_\pf^{n,i-1}\|^2,
\end{equation}
and the errors in chemical potential $\mu$ and $\bm u$ are controlled by the errors in the pressures:
\begin{eqnarray}
    \|e_\mu^{n,i}\|^2&\leq& \frac{LC_\Omega}{2m\tau}\|e_\pf^{n,i-1}\|^2\\
    \|\bm e_{\bm u}^{n,i}\| &\leq& \frac{K_\Omega C_\mathbb{C}\xi d}{c_\mathbb{C}}\| e_\pf^{n,i}\|
\end{eqnarray}
\end{theorem}

\begin{proof}
Start by subtracting equations \eqref{eq:splitch1}--\eqref{eq:splitelastic} from equations \eqref{eq:tdconvexch1}--\eqref{eq:tdconvexelastic} to obtain
\begin{eqnarray}
 \langle e_\pf^{n,i},\eta_\pf \rangle + \tau\langle m \nabla e_\mu^{n,i},\nabla\eta_\pf\rangle &=&0  \label{eq:weakenergych1}\\
 \langle e_\mu^{n,i},\eta_\mu\rangle - \left\langle \gamma\nabla e_\pf^{n,i},\nabla \eta_\mu\right\rangle\nonumber\\ - \left\langle  \Psi'_c(\pf^{n})-\Psi'_c(\pf^{n,i}) -\xi\bm I:\mathbb{C}(\pf^{n-1})\left(\bm\varepsilon(\bm e_{\bm u}^{n,i-1})-\xi e_\pf^{n,i}\bm I\right),\eta_\mu\right\rangle -
 L\langle\pf^{n,i}-\pf^{n,i-1}, \eta_\mu\rangle&=& 0 \label{eq:weakenergych2}\\
  \langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i})- \xi e_\pf^{n,i}\bm I \big),\bm\varepsilon(\bm w)\rangle &=& 0 \label{eq:weakerrorelasticity}.
\end{eqnarray}
Testing with $\eta_\pf = e_\mu^{n,i}$, $\eta_\mu = e_\pf^{n,i}$ and $\bm w = \bm e_{\bm u}^{n,i}$, and subtracting equation \eqref{eq:weakenergych2} from \eqref{eq:weakenergych1} we get
\begin{eqnarray*}
\tau \|m^\frac{1}{2}\nabla e_\mu^{n,i}\|^2 + \gamma\|\nabla e_\pf^{n,i}\|^2 + \langle \Psi'_c(\pf^n)-\Psi_c'(\pf^{n,i}), \pf^n - \pf^{n,i}\rangle \\
- \left\langle\xi\bm I:\mathbb{C}(\pf^{n-1})\left(\bm\varepsilon(\bm e_{\bm u}^{n,i-1})-\xi e_\pf^{n,i}\bm I\right),e_\pf^{n,i}\right\rangle +
 \frac{L}{2}\left(\|e_\pf^{n,i}\|^2 + \|e_\pf^{n,i}- e_\pf^{n,i-1}\|^2 -\|e_\pf^{n,i-1}\|^2\right) &=& 0
\end{eqnarray*}

Using the convexity of $\Psi_c$ and a bit of rearrangements we get 
\begin{eqnarray*}
\tau \|m^\frac{1}{2}\nabla e_\mu^{n,i}\|^2 + \gamma\|\nabla e_\pf^{n,i}\|^2 + C\|e_\pf^{n,i}\|^2 \\ +
 \frac{L}{2}\|e_\pf^{n,i}\|^2 + \frac{L}{2}\|e_\pf^{n,i}- e_\pf^{n,i-1}\|^2   &\leq& \frac{L}{2}\|e_\pf^{n,i-1}\|^2 \\
 && +\langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i-1}) - \bm\varepsilon(\bm e_{\bm u}^{n,i}) + \bm\varepsilon(\bm e_{\bm u}^{n,i})  -\xi e_\pf^{n,i}\bm I\big),\xi e_\pf^{n,i}\bm I\rangle.
\end{eqnarray*}



Distributing we get
\begin{eqnarray}
\tau \|m^\frac{1}{2}\nabla e_\mu^{n,i}\|^2 + \gamma\|\nabla e_\pf^{n,i}\|^2 + C\|e_\pf^{n,i}\|^2\nonumber \\ +
 \frac{L}{2}\|e_\pf^{n,i}\|^2 + \frac{L}{2}\|e_\pf^{n,i}- e_\pf^{n,i-1}\|^2   &\leq& \frac{L}{2}\|e_\pf^{n,i-1}\|^2 
  +\langle \mathbb{C}(\pf^{n-1})\big( \bm\varepsilon(\bm e_{\bm u}^{n,i})  -\xi e_\pf^{n,i}\bm I\big),\xi e_\pf^{n,i}\bm I\rangle \label{eq:beforetricks}\\
 && -\langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\big),\xi e_\pf^{n,i}\bm I\rangle.\nonumber
\end{eqnarray}


From \eqref{eq:weakerrorelasticity} we get by subtracting iteration $i-1$ from $i$ that 
\begin{eqnarray*}
 \langle \mathbb{C}(\pf^{n-1})\left(\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\right), \bm\varepsilon(\bm w)\rangle = 
 \langle \mathbb{C}(\pf^{n-1})\left(e_{\pf}^{n,i} -  e_{\pf}^{n,i-1}\right)\xi\bm I, \bm\varepsilon(\bm w)\rangle 
\end{eqnarray*}
Testing with $\bm w = \bm e_{\bm u}^{n,i} - \bm e_{\bm u}^{n,i-1}$
and using the symmetry, positivity conditions on $\mathbb{C}(s)$: there exists $c>0$ such that 
\begin{equation*}
    \langle\mathbb{C}(s),s\rangle \geq c_\mathbb{C}\|s\|^2,
\end{equation*}
we get 
\begin{eqnarray*}
c_\mathbb{C}\|\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\|^2 \leq 
 \langle \mathbb{C}(\pf^{n-1})\left(e_{\pf}^{n,i} -  e_{\pf}^{n,i-1}\right)\xi\bm I, \bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\rangle 
\end{eqnarray*}
which by an application of Cauchy-Schwarz' inequality yields
\begin{equation}\label{eq:pfboundu}
   \|\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\| \leq\frac{1}{c_\mathbb{C}} 
 \|\mathbb{C}(\pf^{n-1})\left(e_{\pf}^{n,i} -  e_{\pf}^{n,i-1}\right)\xi\bm I\|
\end{equation}

Consider now the term
\begin{equation*}
    -\langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\big),\xi e_\pf^{n,i}\bm I\rangle
\end{equation*}
By Cauchy Schwarz and Young's inequalities we get 
\begin{eqnarray*}
    &-\langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\big),\xi e_\pf^{n,i}\bm I\rangle\\
    &\leq \frac{\delta}{2}\|\mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\big)\|^2 + \frac{1}{2\delta}\| \xi e_\pf^{n,i}\bm I \|^2
\end{eqnarray*}

Using the boundedness of $\mathbb{C}$ and \eqref{eq:pfboundu} we get 


\begin{eqnarray*}
    &-\langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\big),\xi e_\pf^{n,i}\bm I\rangle\\
    &\leq \frac{\delta C_\mathbb{C}^2}{2c_\mathbb{C}^2} \|\mathbb{C}(\pf^{n-1})\left(e_{\pf}^{n,i} -  e_{\pf}^{n,i-1}\right)\xi\bm I\|^2 + \frac{1}{2\delta}\| \xi e_\pf^{n,i}\bm I \|^2
\end{eqnarray*}
Using again the boundedness of $\mathbb{C}$ and choosing $\delta = \frac{1}{2d^2C\xi^2}$ we get
\begin{eqnarray*}
    &-\langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm e_{\bm u}^{n,i}) - \bm\varepsilon(\bm e_{\bm u}^{n,i-1})\big),\xi e_\pf^{n,i}\bm I\rangle\\
    &\leq \frac{C_\mathbb{C}^3}{4Cc_\mathbb{C}^2} \|\mathbb{C}(\pf^{n-1})\left(e_{\pf}^{n,i} -  e_{\pf}^{n,i-1}\right)\xi\bm I\|^2 + C\| e_\pf^{n,i}\|^2
\end{eqnarray*}

From equation \eqref{eq:beforetricks} we then get by choosing $L\geq  \frac{C_\mathbb{C}^3}{4Cc_\mathbb{C}^2}$
\begin{eqnarray*}
\tau \|m^\frac{1}{2}\nabla e_\mu^{n,i}\|^2 + \gamma\|\nabla e_\pf^{n,i}\|^2  + \frac{L}{2}\|e_\pf^{n,i}\|^2 &\leq& \frac{L}{2}\|e_\pf^{n,i-1}\|^2 
  +\langle \mathbb{C}(\pf^{n-1})\big( \bm\varepsilon(\bm e_{\bm u}^{n,i})  -\xi e_\pf^{n,i}\bm I\big),\xi e_\pf^{n,i}\bm I\rangle
\end{eqnarray*}
If now $\bm w$ can be chosen such that \todo{Quite sure that this is exactly what we had in the optimization fixed stress paper, where an inf-sup stable discretization (e.g., P2 for elasticity and P1 for flow) is required.}
\begin{equation}
    \langle q, \bm \varepsilon(\bm w)\rangle = \langle q , \xi e_\pf^{n,i}\bm I\rangle,
\end{equation}
which is equivalent to 
\begin{equation}
    \langle q, \nabla\cdot \bm w\rangle = \langle q ,  e_\pf^{n,i}\rangle,
\end{equation}
then equation \eqref{eq:weakerrorelasticity} together with Poincar\'e's inequality gives the contraction
\begin{equation}
\left(\frac{\gamma}{C_\Omega}+\frac{L}{2}\right)\|e_\pf^{n,i}\|^2 \leq \frac{L}{2}\|e_\pf^{n,i-1}\|^2.
\end{equation}

Moreover, the error in the chemical potential is controlled by the error in the phase-field
\begin{equation}
    \tau\|m^\frac{1}{2}\nabla e_\mu^{n,i}\|^2\leq \frac{L}{2}\|e_\pf^{n,i-1}\|^2,
\end{equation}
and thereby with Poincar\'e's inequality tends to zero.

By testing equation \eqref{eq:weakerrorelasticity} with $\bm w = \bm e_{\bm u}^{n,i}$ and using the properties of $\mathbb{C}$ and Cauchy-Schwarz we get that
\begin{equation*}
      \langle \mathbb{C}(\pf^{n-1})\bm\varepsilon(\bm e_{\bm u}^{n,i}),\bm\varepsilon(\bm e_{\bm u}^{n,i})\rangle = \langle \mathbb{C}(\pf^{n-1}) \xi e_\pf^{n,i}\bm I,\bm\varepsilon(\bm e_{\bm u}^{n,i})\rangle
\end{equation*}
\begin{equation*}
     c_\mathbb{C}\|\bm\varepsilon(\bm e_{\bm u}^{n,i})\|^2 \leq C_\mathbb{C}\|\xi e_\pf^{n,i}\bm I\|\|\bm\varepsilon(\bm e_{\bm u}^{n,i})\|
\end{equation*}
\begin{equation*}
     \|\bm\varepsilon(\bm e_{\bm u}^{n,i})\| \leq \frac{C_\mathbb{C}\xi d}{c_\mathbb{C}}\| e_\pf^{n,i}\|
\end{equation*}
and by Korn's inequality we also get that $\bm e_{\bm u}^{n,i} \to 0$ as $i\to \infty$.



We can here also do a splitting between convex and nonconvex parts of the energy to get purely convex minimization problems
\begin{eqnarray}
    \pf^n\!\!\!\! &=&\!\!\!\! \argmin_{s} \left\{\frac{\|s \|_{H^{-1}_{m}(\Omega)}^2}{2} + \tau\left(\mathcal{E}_c(s, \bm u^n, \pf^{n-1}) - \int_\Omega \Psi_e'(\pf^{n-1}) s \; dx  \right)+ \tau\langle R, s\rangle_{H^{-1}_m(\Omega)} +\langle z^{n-1}, s\rangle_{H^{-1}_m(\Omega)}\right\} \\
    \bm u^n\!\!\!\! &=&\!\!\!\!\argmin_{\bm w} \left\{\mathcal{E}_c(\pf^n, \bm w, \pf^{n-1}) +  \langle\bm f,\bm w\rangle_{L^2(\Omega)} \right\},
\end{eqnarray}
where 
\begin{equation}
    \mathcal{E}_c(s, \bm u^n, \pf^{n-1}) = \int_\Omega \Psi_c(s) + \gamma\frac{|\nabla s|^2}{2} + \frac{1}{2}\left(\bm\varepsilon(\bm u^n) - \xi s \bm I\right)\mathbb{C}(\pf^{n-1})\left(\bm \varepsilon(\bm u^n) - \xi s \bm I \right) \; dx.
\end{equation}
Computing optimality conditions we get the time-discrete system of equations
\begin{eqnarray}
 \langle \pf^n,\eta_\pf \rangle + \tau\langle m(\pf^n) \nabla\mu^n,\nabla\eta_\pf\rangle - \tau\langle  R^n ,\eta_\pf\rangle - \langle\pf^{n-1},\eta_\pf \rangle&=&0 \label{eq:tdconvexch1} \\
 \langle \mu^n,\eta_\mu\rangle - \left\langle \gamma\nabla\pf^n,\nabla \eta_\mu\right\rangle - \left\langle  \Psi'_c(\pf^n) - \Psi'_e(\pf^{n-1})  -\xi\bm I:\mathbb{C}(\pf^{n-1})\left(\bm\varepsilon(\bm u^n)-\xi \pf^n\bm I\right),\eta_\mu\right\rangle &=& 0 \label{eq:tdconvexch2}\\
  \langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm u^n)- \xi\pf^n\bm I) \big),\bm\varepsilon(\bm w)\rangle + \langle \bm f^n,\bm w\rangle &=& 0 \label{eq:tdconvexelastic}
\end{eqnarray}

\subsection{Linearization and splitting}
The system of equations \eqref{eq:tdconvexch1}--\eqref{eq:tdconvexelastic} is still a nonlinear system of equations to be solved in each time step. Although the most natural approach might be to apply the Newton method, one could encounter some trouble with local convergence, especially in equation \eqref{eq:tdconvexelastic}. Therefore, we suggest to apply a decoupling method to solve the equations:
Given $L>0$, and $(\pf^{n-1}, \pf^{n,i-1}, \bm u^{n,i-1})$, find $(\pf^{n,i}, \mu^{n,i} \bm u^{n,i})$ such that 
\begin{eqnarray}
 \langle \pf^{n,i},\eta_\pf \rangle + \tau\langle m(\pf^{n,i}) \nabla\mu^{n,i},\nabla\eta_\pf\rangle -\tau \langle  R^n ,\eta_\pf\rangle - \langle\pf^{n-1},\eta_\pf \rangle&=&0 \label{eq:splitch1} \\
 \langle \mu^{n,i},\eta_\mu\rangle - \left\langle \gamma\nabla\pf^{n,i},\nabla \eta_\mu\right\rangle\nonumber\\ - \left\langle  \Psi'_c(\pf^{n,i}) - \Psi'_e(\pf^{n-1})  -\xi\bm I:\mathbb{C}(\pf^{n-1})\left(\bm\varepsilon(\bm u^{n,i-1})-\xi \pf^{n,i}\bm I\right),\eta_\mu\right\rangle -
 L\langle\pf^{n,i}-\pf^{n,i-1}, \eta_\mu\rangle&=& 0 \label{eq:splitch2}\\
  \langle \mathbb{C}(\pf^{n-1})\big(\bm\varepsilon(\bm u^{n,i})- \xi\pf^{n,i}\bm I) \big),\bm\varepsilon(\bm w)\rangle + \langle \bm f^n,\bm w\rangle &=& 0 \label{eq:splitelastic},
\end{eqnarray}
where equation \eqref{eq:splitch1}-\eqref{eq:splitch2} is solved first to find $\pf^{n,i}$ before we solve equation \eqref{eq:splitelastic} to get an updated solution for $\bm u^{n,i}$. Notice that the Cahn-Hilliard subsystem \eqref{eq:splitch1}--\eqref{eq:splitch2} still is a nonlinear system of equations, and there are several choices here. As a first suggestion we suggest to solve it with the Newton method, which is known to theoretically converge for this problem using the techniques of \todo{cite paper with convex concave newton convergence.}, and then define $\pf^{n,i}$, $\mu^{n,i}$ as the solution after the Newton method has converged to satisfactory precision. Alternatively one could consider to linearize the equation with the Newton method and only solve the equations once before switching to solve elasticity \eqref{eq:splitelastic}.
% \subsection{Convex-concave splitting methods}
% An important aspect when considering solution strategies to Cahn-Hilliard-type equations is how to deal with the non-convex double-well potential. Evaluating it implicitly is typically not feasible as one might encounter stability issues (not convergence of the linearization method). A popular remedy is to apply convex-concave splitting methods in time and there is quite a lot of theory available already\todo{add references}. The classical work of Eyre \cite{eyre1998} suggests to split the double-well into two terms $\Psi_c(\pf) - \Psi_e(\pf)$ that are both convex and evaluate $\Psi_c(\pf^n)$ implicitly  and $\Psi_e(\pf^{n-1})$ explicitly. For the double-well in this work Eyre's method suggests to choose
% \begin{equation}
%     \Psi(\pf) =  (\pf^2-1)^2 = (\pf^4+1) - 2\pf^2 =: \Psi_c(\pf) - \Psi_e(\pf). 
% \end{equation}
% There exists several other works considering the treatment of the double-well potential in the literature.

% For the Cahn-Larch\'e equations, however, we also have the non-convex nonlinearity related to the elastic energy $\mathcal{E}_\mathrm{e}$. We will consider several ways to deal with this term, but we start with the simpler case of homogeneous elasticity tensor, where $\mathcal{E}_\mathrm{e}$ is convex, and the coupling between phase-field and elasticity is linear.



\subsection{Minimization structure of the Cahn-Larch\'e equations}
The Cahn-Larch\'e equations follow a generalized gradient flow structure \cite{storvikCHB}, and therefore also has an inherent minimization structure. This is going to be valuable when considering solution algorithms to the system. 
To put the equations into the minimization framework, we first define the $H^{-1}_m(\Omega)$ inner-product, which is naturally related to conservative diffusion processes. 
\begin{definition}
    Let $f_1 = -\nabla \cdot m^{-1}\nabla g_1$, and $f_2 =-\nabla \cdot m^{-1}\nabla g_2$. The $H^{-1}_m(\Omega)$ inner-product is defined as \begin{equation}
        \langle f_1, f_2 \rangle_{H^{-1}_m(\Omega)} = \left\langle m^{-\frac{1}{2}}\nabla g_1, m^{-\frac{1}{2}}\nabla g_2 \right\rangle_{L^2(\Omega)} = \langle f_1, g_2 \rangle_{L^2(\Omega)},
    \end{equation}
    and the induced norm is denoted by $$\|f_1\|_{H^{-1}_m(\Omega)} = \langle f_1,f_1\rangle^\frac{1}{2}_{H^{-1}_m(\Omega)}.$$
\end{definition}

For the Cahn-Larch\'e system we can then see that the equations appear as optimality conditions to the minimization problem

\begin{eqnarray}\label{eq:CHEContinuousGradientFlowMinimization1}
    \partial_t \pf &=& \argmin_{s} \left\{\frac{\|s \|_{H^{-1}_{m}(\Omega)}^2}{2} + \langle\delta_{\pf}\mathcal{E}(\pf, \bm u),s\rangle_{L^2(\Omega)} + \langle R, s\rangle_{H^{-1}_m(\Omega)}  \right\}\\
    \bm u &=& \argmin_{\bm w} \left\{ \mathcal{E}(\pf, \bm w) +  \langle\bm f,\bm w\rangle_{L^2(\Omega)} \right\} \label{eq:CHEContinuousGradientFlowMinimization2}
\end{eqnarray}

\begin{remark}
Both the heterogeneous \eqref{eq:ch1}--\eqref{eq:elasticity} and the homogeneous \eqref{eq:homoch1}--\eqref{eq:homoelasticity} Cahn-Larch\'e equations are generalized gradient flows, and can be formulated as the minimization problem \eqref{eq:CHEContinuousGradientFlowMinimization1}--\eqref{eq:CHEContinuousGradientFlowMinimization2}, by choosing the elasticity tensor $\mathbb{C}$ in the free energy \eqref{eq:freeenergy} either dependent or independent on $\pf$.
\end{remark}

